Do LLMs Build World Models From Text? A Multilingual Diagnostic of Spatial Reasoning

Whether large language models (LLMs) construct internal spatial world models from pure-text descriptions remains contested, and whether such capabilities transfer across languages has not been systematically studied. We introduce MentalMap, a multilingual diagnostic benchmark with a six-level capability hierarchy (L0-L5) spanning atomic spatial facts to generative world-graph construction, together with four diagnostic axes probing frame of reference, reading-direction bias, reasoning-effort allocation, and hallucination. MentalMap is built from 100 ProcTHOR household scenes, covers eight typologically diverse languages plus a structured-text control, and contains 39 task families across 1,950 evaluation cells. Evaluating thirteen LLMs across scales and model families, we identify a universal L3 reasoning cliff: no model retains even half of its L0 performance on viewpoint reasoning once baseline atomic accuracy exceeds 40%. The cliff persists across languages, scales, and prompting strategies, while structured-output failures and reasoning patterns vary substantially across models. Human evaluation under the identical pure-text protocol reproduces the same failure pattern, suggesting that the bottleneck arises from text-only working memory constraints rather than being specific to current LLM architectures. Our findings reframe pure-text spatial reasoning as a multi-axis world-modeling problem and motivate multimodal and scratchpad-augmented reasoning as future directions.

==> figures/pipeline_staircase.tex <==
% =============================================================================
% MERGED FIGURE v2: data pipeline (left) + capability staircase examples (right).
% Adds: per-stage line-art icons, hand-drawn TikZ flag chips for 8 languages,
% and tightened spacing between the two halves.
% =============================================================================
\begin{figure*}[t]
\centering

\definecolor{stageGray}{HTML}{F1EFE8}\definecolor{stageGrayBd}{HTML}{888780}
\definecolor{stagePurple}{HTML}{EEEDFE}\definecolor{stagePurpleBd}{HTML}{7F77DD}
\definecolor{stageTeal}{HTML}{E1F5EE}\definecolor{stageTealBd}{HTML}{1D9E75}
\definecolor{stageCoral}{HTML}{FAECE7}\definecolor{stageCoralBd}{HTML}{D85A30}
\definecolor{stageAmber}{HTML}{FAEEDA}\definecolor{stageAmberBd}{HTML}{BA7517}
\definecolor{lvl0}{HTML}{F1EFE8}\definecolor{lvl0Bd}{HTML}{888780}
\definecolor{lvl1}{HTML}{E6F1FB}\definecolor{lvl1Bd}{HTML}{378ADD}
\definecolor{lvl2}{HTML}{E1F5EE}\definecolor{lvl2Bd}{HTML}{1D9E75}
\definecolor{lvl3}{HTML}{FAEEDA}\definecolor{lvl3Bd}{HTML}{BA7517}
\definecolor{lvl4}{HTML}{FAECE7}\definecolor{lvl4Bd}{HTML}{D85A30}
\definecolor{lvl5}{HTML}{EEEDFE}\definecolor{lvl5Bd}{HTML}{7F77DD}
\definecolor{flagRed}{HTML}{D32F2F}
\definecolor{flagBlue}{HTML}{1565C0}
\definecolor{flagYellow}{HTML}{FFD600}
\definecolor{flagGreen}{HTML}{2E7D32}
\definecolor{flagBlack}{HTML}{212121}
\definecolor{flagWhite}{HTML}{FFFFFF}

\begin{adjustbox}{center, max width=\textwidth}
\begin{tikzpicture}[
    font=\scriptsize,
    every node/.style={align=center, inner sep=4pt, line width=0.4pt, rounded corners=2pt},
    pstage/.style={
        rectangle, draw, line width=0.4pt, rounded corners=3pt,
        text width=5.5cm, minimum height=8mm, align=center, font=\scriptsize
    },
    pstagebig/.style={
        rectangle, draw, line width=0.4pt, rounded corners=3pt,
        text width=5.5cm, minimum height=12mm, align=center, font=\scriptsize
    },
    psub/.style={
        rectangle, draw, line width=0.4pt, rounded corners=3pt,
        text width=1.55cm, minimum height=8mm, align=center, font=\scriptsize
    },
    levelbox/.style={
        rectangle, draw, line width=0.4pt, rounded corners=3pt,
        text width=1.9cm, minimum height=9mm, align=center, font=\scriptsize
    },
    exbox/.style={
        rectangle, draw, line width=0.3pt, rounded corners=2pt,
        text width=5.4cm, minimum height=9mm, align=left, font=\scriptsize,
        fill=white!50!gray!4
    },
    arr/.style={-{Stealth[length=1.8mm,width=1.4mm]}, line width=0.4pt, draw=black!55},
    icon/.style={line width=0.4pt, draw=black!60},
]

% ============ LEFT COLUMN: pipeline ============
\node[pstage, fill=stageGray, draw=stageGrayBd!70] (s1) at (0,0)
    {\textbf{Stage 1 \textbar{} Scene grounding} \\[0.3mm]
     \scriptsize ProcTHOR 100 houses $+$ AI2-THOR \\ \scriptsize 17 high-level actions};
\begin{scope}[shift={(s1.east)}, xshift=-7mm, icon]
  \draw (-3mm,-2.2mm) -- (-3mm,1mm) -- (-0.5mm,2.5mm) -- (2mm,1mm) -- (2mm,-2.2mm) -- cycle;
  \draw (-1.5mm,-2.2mm) rectangle (-0.3mm,0);
  \draw[-{Stealth[length=1mm,width=0.8mm]}] (3mm,-0.5mm) arc (-90:90:1mm);
\end{scope}

% Stage 2 — three causal artifacts: initial scene -> action sequence -> state log
% Each box has a clearer name + a one-line role description, and they are
% connected by an in-line causal arrow showing the temporal relationship.
\node[psub, fill=stagePurple, draw=stagePurpleBd!70, below=10mm of s1.south, anchor=north, xshift=-2.1cm,
      text width=1.45cm, minimum height=11mm] (s2a)
    {\textbf{World state} \\[0.2mm] \scriptsize \textit{(t\,=\,0)} \\ \scriptsize objects, \\ \scriptsize attributes};
\node[psub, fill=stagePurple, draw=stagePurpleBd!70, right=6mm of s2a,
      text width=1.45cm, minimum height=11mm] (s2b)
    {\textbf{Trajectory} \\[0.2mm] \scriptsize \textit{ordered actions} \\ \scriptsize with pre/post \\ \scriptsize conditions};
\node[psub, fill=stagePurple, draw=stagePurpleBd!70, right=6mm of s2b,
      text width=1.45cm, minimum height=11mm] (s2c)
    {\textbf{Transition log} \\[0.2mm] \scriptsize \textit{step-by-step} \\ \scriptsize state changes \\ \scriptsize (before$\,\to\,$after)};

% horizontal causal arrows (t=0 -> process -> diff), made visible by the 6mm gap
\draw[-{Stealth[length=2mm,width=1.6mm]}, line width=0.5pt, draw=black!60]
    (s2a.east) -- (s2b.west);
\draw[-{Stealth[length=2mm,width=1.6mm]}, line width=0.5pt, draw=black!60]
    (s2b.east) -- (s2c.west);

\node[font=\scriptsize\itshape, text=black!55, anchor=south] at ($(s2b.north)+(0,0.1cm)$)
    {Stage 2 \textbar{} Canonical scene formalization};

\node[pstage, fill=stageTeal, draw=stageTealBd!70, below=11mm of s2b.south, anchor=north] (s3)
    {\textbf{Stage 3 \textbar{} Task generation} \\[0.3mm]
     \scriptsize 36 base tasks across the \\ \scriptsize L0--L5 capability staircase $\rightarrow$};
\begin{scope}[shift={(s3.east)}, xshift=-7mm, icon]
  \draw (-3.5mm,-2.5mm) -- (-2mm,-2.5mm) -- (-2mm,-1mm) -- (-0.5mm,-1mm) -- (-0.5mm,0.5mm) -- (1mm,0.5mm) -- (1mm,2mm) -- (2.5mm,2mm);
\end{scope}

% Stage 4 with flag row above
\node[pstagebig, fill=stageCoral, draw=stageCoralBd!70, below=11mm of s3.south, anchor=north] (s4)
    {\textbf{Stage 4 \textbar{} Multilingual rendering $\times$ axes} \\[0.5mm]
     \scriptsize 8 languages (flags above) $+$ structured control \\ \scriptsize 3 frames $\cdot$ 2 RTL orders $\cdot$ 4 styles $\cdot$ 8 views};

\newcommand{\flagchip}[3]{%
  \begin{scope}[shift={#1}]
    #3
    \draw[line width=0.2pt, draw=black!50] (-2.5mm,-1.5mm) rectangle (2.5mm,1.5mm);
    \node[font=\tiny, anchor=north, inner sep=0.5pt, text=black!70] at (0,-1.8mm) {#2};
  \end{scope}
}
\coordinate (flagrow) at ($(s4.north)+(0,4mm)$);
% en
\flagchip{($(flagrow)+(-24.5mm,0)$)}{en}{%
  \fill[flagBlue] (-2.5mm,-1.5mm) rectangle (2.5mm,1.5mm);
  \draw[white, line width=0.55pt] (-2.5mm,-1.5mm) -- (2.5mm,1.5mm);
  \draw[white, line width=0.55pt] (-2.5mm,1.5mm) -- (2.5mm,-1.5mm);
  \fill[white] (-0.55mm,-1.5mm) rectangle (0.55mm,1.5mm);
  \fill[white] (-2.5mm,-0.45mm) rectangle (2.5mm,0.45mm);
  \fill[flagRed] (-0.25mm,-1.5mm) rectangle (0.25mm,1.5mm);
  \fill[flagRed] (-2.5mm,-0.2mm) rectangle (2.5mm,0.2mm);
}
% zh
\flagchip{($(flagrow)+(-17.5mm,0)$)}{zh}{%
  \fill[flagRed] (-2.5mm,-1.5mm) rectangle (2.5mm,1.5mm);
  \node[star, star points=5, star point ratio=2.5, fill=flagYellow, draw=flagYellow,
        minimum size=1.6mm, inner sep=0pt] at (-1.2mm,0.5mm) {};
  \node[star, star points=5, star point ratio=2.5, fill=flagYellow, draw=flagYellow,
        minimum size=0.6mm, inner sep=0pt] at (0.3mm,0.95mm) {};
}
% ja
\flagchip{($(flagrow)+(-10.5mm,0)$)}{ja}{%
  \fill[flagWhite] (-2.5mm,-1.5mm) rectangle (2.5mm,1.5mm);
  \fill[flagRed] (0,0) circle (0.85mm);
}
% ko
\flagchip{($(flagrow)+(-3.5mm,0)$)}{ko}{%
  \fill[flagWhite] (-2.5mm,-1.5mm) rectangle (2.5mm,1.5mm);
  \fill[flagRed] (0,0) circle (0.85mm);
  \begin{scope} \clip (0,0) circle (0.85mm); \fill[flagBlue] (-1mm,-1mm) rectangle (1mm,0); \end{scope}
}
% es
\flagchip{($(flagrow)+(3.5mm,0)$)}{es}{%
  \fill[flagRed] (-2.5mm,-1.5mm) rectangle (2.5mm,1.5mm);
  \fill[flagYellow] (-2.5mm,-0.75mm) rectangle (2.5mm,0.75mm);
}
% ar
\flagchip{($(flagrow)+(10.5mm,0)$)}{ar}{%
  \fill[flagGreen] (-2.5mm,-1.5mm) rectangle (2.5mm,1.5mm);
  \draw[white, line width=0.4pt] (-1.5mm,0) -- (1.5mm,0);
}
% th
\flagchip{($(flagrow)+(17.5mm,0)$)}{th}{%
  \fill[flagRed] (-2.5mm,-1.5mm) rectangle (2.5mm,1.5mm);
  \fill[flagWhite] (-2.5mm,-0.9mm) rectangle (2.5mm,0.9mm);
  \fill[flagBlue] (-2.5mm,-0.4mm) rectangle (2.5mm,0.4mm);
}
% de
\flagchip{($(flagrow)+(24.5mm,0)$)}{de}{%
  \fill[flagBlack] (-2.5mm,0.5mm) rectangle (2.5mm,1.5mm);
  \fill[flagRed] (-2.5mm,-0.5mm) rectangle (2.5mm,0.5mm);
  \fill[flagYellow] (-2.5mm,-1.5mm) rectangle (2.5mm,-0.5mm);
}

\node[pstage, fill=stageGray, draw=stageGrayBd!70, below=8mm of s4.south, anchor=north] (s5)
    {\textbf{Stage 5 \textbar{} Model evaluation} \\[0.3mm]
     \scriptsize 9 models: 3 closed-source $\cdot$ 6 open-weight};
\begin{scope}[shift={(s5.east)}, xshift=-7mm, icon]
  \draw (-2.5mm,1.2mm) rectangle (2.5mm,2.4mm);
  \draw (-2.5mm,-0.6mm) rectangle (2.5mm,0.6mm);
  \draw (-2.5mm,-2.4mm) rectangle (2.5mm,-1.2mm);
\end{scope}

\node[pstage, fill=stageAmber, draw=stageAmberBd!70, below=8mm of s5.south, anchor=north] (s6)
    {\textbf{Stage 6 \textbar{} Per-axis metrics} \\[0.3mm]
     \scriptsize pass rate $\cdot$ frame-shift drop $\cdot$ anchor dist. \\ \scriptsize reasoning delta $\cdot$ node/edge F1};
\begin{scope}[shift={(s6.east)}, xshift=-7mm, icon]
  \draw (-3mm,-2.2mm) rectangle (-1.8mm,0mm);
  \draw (-1.2mm,-2.2mm) rectangle (0mm,1.8mm);
  \draw (0.6mm,-2.2mm) rectangle (1.8mm,-1mm);
  \draw (2.4mm,-2.2mm) rectangle (3.6mm,0.8mm);
\end{scope}

% arrows
\draw[arr] (s1.south) -- (s2a.north);   % Stage 1 -> first artifact (t=0)
% s2a -> s2b -> s2c arrows already drawn above (causal chain)
\draw[arr] (s2a.south) -- (s3.north -| s2a.south);
\draw[arr] (s2b.south) -- (s3.north -| s2b.south);
\draw[arr] (s2c.south) -- (s3.north -| s2c.south);
\draw[arr] (s3.south) -- (s4.north);
\draw[arr] (s4.south) -- (s5.north);
\draw[arr] (s5.south) -- (s6.north);

% ============ RIGHT COLUMN: staircase ============
\coordinate (rightx) at (6.8,0);

\node[levelbox, fill=lvl0, draw=lvl0Bd!70, anchor=north west] (l0) at ($(rightx)+(0,0)$)
    {\textbf{L0 Atomic} \\ \scriptsize 5 tasks};
\node[exbox, anchor=west] (l0e) at ($(l0.east)+(0.2cm,0)$)
    {\textit{``Is there an apple in the kitchen?''} \\ \textit{``How many apples are on the CounterTop?''}};

\node[levelbox, fill=lvl1, draw=lvl1Bd!70, anchor=north west] (l1) at ($(l0.south west)+(0,-0.3cm)$)
    {\textbf{L1 Anchor} \\ \scriptsize 5 tasks};
\node[exbox, anchor=west] (l1e) at ($(l1.east)+(0.2cm,0)$)
    {\textit{``Where is the apple?''} \,/\, \textit{``Is the knife on the CounterTop?''}};

\node[levelbox, fill=lvl2, draw=lvl2Bd!70, anchor=north west] (l2) at ($(l1.south west)+(0,-0.3cm)$)
    {\textbf{L2 Multi-} \\ \textbf{Object} \\ \scriptsize 4 tasks};
\node[exbox, anchor=west] (l2e) at ($(l2.east)+(0.2cm,0)$)
    {\textit{``The apple is on the CounterTop. The CounterTop is in the Kitchen. Where is the apple?''}};

\node[levelbox, fill=lvl3, draw=lvl3Bd!70, anchor=north west] (l3) at ($(l2.south west)+(0,-0.3cm)$)
    {\textbf{L3 Viewpoint} \\ \scriptsize 5 tasks};
\node[exbox, anchor=west] (l3e) at ($(l3.east)+(0.2cm,0)$)
    {\textit{``You face north; the Fridge is on your right. After turning 90$^\circ$ clockwise, what is in front of you?''}};

\node[levelbox, fill=lvl4, draw=lvl4Bd!70, anchor=north west] (l4) at ($(l3.south west)+(0,-0.3cm)$)
    {\textbf{L4 Dynamic} \\ \scriptsize 13 tasks \\ \scriptsize (a/b/c)};
\node[exbox, anchor=west] (l4e) at ($(l4.east)+(0.2cm,0)$)
    {\textit{``Execute these 5 actions in order. Where are the apple and the knife now?''} \\
     {\scriptsize\color{black!55}representative: L4c multi-step chain}};

\node[levelbox, fill=lvl5, draw=lvl5Bd!70, anchor=north west] (l5) at ($(l4.south west)+(0,-0.3cm)$)
    {\textbf{L5 Generative} \\ \textbf{World-graph} \\ \scriptsize 4 tasks (a/b/c/d)};
\node[exbox, anchor=west] (l5e) at ($(l5.east)+(0.2cm,0)$)
    {\textit{``Output a JSON world graph of the kitchen.''} \\
     {\scriptsize\color{black!55}representative: L5a static graph}};

% bracket connecting Stage 3 to the staircase block
\coordinate (l0top) at ($(l0.north west)+(0,0.05cm)$);
\coordinate (l5bot) at ($(l5.south west)+(0,-0.05cm)$);
\draw[line width=0.5pt, draw=black!45]
    (l0top) -- ($(l0top)+(-0.3cm,0)$) -- ($(l5bot)+(-0.3cm,0)$) -- (l5bot);
\draw[arr] (s3.east) -- ($(s3.east)+(0.4cm,0)$)
    |- ($(l0top)!0.5!(l5bot)+(-0.3cm,0)$);

% Increasing-demand arrow left of bracket
\draw[line width=0.5pt, draw=black!40, ->]
    ($(l0top)+(-0.55cm,0)$) -- ($(l5bot)+(-0.55cm,0)$);
\node[font=\scriptsize\itshape, rotate=90, text=black!55, anchor=south]
    at ($(l0top)!0.5!(l5bot)+(-0.63cm,0)$) {Increasing spatial demand};

\node[font=\scriptsize\bfseries, anchor=south west] at ($(l0.north west)+(0,0.12cm)$)
    {Capability staircase \textbar{} representative task (English rendering)};

\end{tikzpicture}
\end{adjustbox}

\caption{
\label{fig:pipeline_staircase}
\textbf{\mentalmap{} data-generation pipeline and capability staircase.}
\emph{Left:} the six-stage generation pipeline. A ProcTHOR house and a sampled
AI2-THOR action sequence (Stage~1) are decomposed into three
language-independent canonical artifacts---the initial \emph{world state}, the
action \emph{trajectory}, and the per-step \emph{transition log} (Stage~2). Stage~3 instantiates 36 base tasks organized along the
L0--L5 capability staircase; each base case is then rendered in eight
typologically diverse languages (English, Mandarin, Japanese, Korean, Spanish,
Arabic, Thai, German) plus a structured-text control and crossed with diagnostic
axes (Stage~4), evaluated on 9 models (Stage~5), and scored with per-axis
metrics (Stage~6). \emph{Right:} the capability staircase, with one
representative task per level (English rendering shown). L0--L2 probe
\emph{static comprehension} of increasing compositional depth; L3 marks the
boundary to \emph{active spatial reasoning} with viewpoint and frame-of-reference tasks;
L4 targets \emph{dynamic state update} under lengthening action horizons; L5 requires
\emph{generative structured world-graph output}. Per-level evaluation metrics
and diagnostic intent are detailed in Section~\ref{sec:bd_axes} and Appendix~\ref{sec:app_design_details}.
}
\end{figure*}


==> sections/04_experimental_setup.tex <==
\section{Experimental Setup}
\label{sec:experimental_setup}

% TODO(Mill): Fill in once final model list and infrastructure decisions are locked.
% Current draft assumes 17-model evaluation; adjust if scope changes.

\subsection{Models Evaluated}
\label{sec:exp_models}

We evaluate 17 language models spanning four families and three reasoning regimes.

\noindent\textbf{Frontier closed-source.} GPT-5, GPT-5-mini, GPT-4o \citep{openai2024gpt4o}, Claude 3.7 Sonnet (with extended thinking enabled and disabled, reported separately) \citep{anthropic2025claude37}, Gemini 2.5 Pro \citep{google2025gemini25}.

\noindent\textbf{Frontier reasoning models.} OpenAI o3 \citep{openai2025o3}, DeepSeek-R1 \citep{deepseek2025r1}, DeepSeek-R1-Distill-Qwen-32B \citep{deepseek2025r1}, QwQ-32B-Preview \citep{qwen2024qwq}, Qwen3-32B with thinking mode \citep{qwen2025qwen3}.

\noindent\textbf{Open-weight base models.} Llama-3.1 70B \citep{grattafiori2024llama3}, Llama-3.1 8B, Qwen2.5-72B-Instruct \citep{qwen2024qwen25}, Qwen2.5-7B-Instruct, Mistral-Large-2 \citep{mistral2024large2}, GLM-4-Plus \citep{glm2024glm4}.

\noindent\textbf{Multilingual-emphasis models.} Aya-Expanse-32B \citep{cohere2024aya}, Jais-70B \citep{jais2023}.

\subsection{Prompting Protocols}
\label{sec:exp_protocols}

For each task we evaluate four prompting strategies: zero-shot, four-shot, chain-of-thought (CoT) \citep{wei2022chain}, and structured-guidance (SG) prompting following \citep{premsri2025forest}. For long-reasoning models we additionally enable thinking mode and record thinking traces.

For diagnostic axes we use specialized protocols: frame-of-reference variants are presented zero-shot to avoid in-context FoR contamination; RTL bias is measured on free-form generation rather than multiple choice; belief-revision uses three-turn dialogues with controlled conflict injection; hallucination detection uses open-ended scene description with ground-truth scene-graph comparison.

\subsection{Evaluation Infrastructure}
\label{sec:exp_infrastructure}

All evaluations run on standardized infrastructure with deterministic decoding (temperature 0 for non-thinking models; default sampling for thinking models per their published recommendations). For closed-source models we use official APIs; for open-weight models we use vLLM \citep{vllm2023} on 8$\times$A100 80GB nodes. Total evaluation cost approximately 2{,}400 GPU-hours plus API costs detailed in Appendix~\ref{sec:appendix}.

% PLACEHOLDER: Add table with model list, parameter counts, and key configuration once final.


==> sections/05_results.tex <==
\section{Results}
\label{sec:results}

This section reports seven findings derived from the nine-model, eight-language
evaluation. Section~\ref{sec:res_staircase} establishes the main staircase
result; Section~\ref{sec:res_l3_cliff}--\ref{sec:res_hallucination} expand on
diagnostic-axis sub-findings.

\subsection{Capability Staircase Across Languages}
\label{sec:res_staircase}

\input{tables/main_results}

Table~\ref{tab:main_results} reports composite scores per (model, language,
level) for the three highest staircase levels. Two patterns dominate. First,
\textbf{the staircase is non-monotonic}: all nine models show a sharp drop at
L3 (viewpoint) and a partial recovery at L4--L5. GPT-4o's English scores
illustrate the shape: 32.4 / 52.4 / 93.3 (L3/L4/L5). The L5 number reflects
partial-credit graph F1; the strict pass rate is far lower, as we discuss in
Section~\ref{sec:res_metric}. Second, \textbf{cross-language consistency is
low}: the gap between best and worst language ranges from 14 points (GPT-4o)
to 25 points (Falcon3-10B), with Arabic and Thai consistently weakest.

The combined-cross-axis Table~\ref{tab:cross_axis_summary} provides three
complementary views that we expand on in the next three subsections: an
L3 sub-task breakdown (left block), reasoning-prompt deltas (middle block),
and the L5 node/edge F1 dissociation (right block).

\input{tables/cross_axis_summary}

\subsection{The L3 Cliff Is Sub-Task Structured, Not Uniform}
\label{sec:res_l3_cliff}

The headline ``L3 cliff'' finding requires unpacking. The left block of
Table~\ref{tab:cross_axis_summary} shows that the five L3 sub-tasks are
\emph{not} uniformly hard. Two sub-tasks---\texttt{globalToView} and
\texttt{viewpointShift}---are universally near-zero across all open-weight
models (typically 0\% or below 5\%). A third, \texttt{rotation}, is partially
solvable by some models (Qwen2.5-7B 25.6\%, Gemma 36.7\%) but at chance level
for others. A fourth, \texttt{viewToGlobal}, is solvable in English by GPT-4o
(45.4\%) and Falcon3 (41.1\%) but collapses in non-English variants. The
remaining sub-task, \texttt{rotationCheck}, is a boolean consistency check
that admits substantial guessing: Qwen2.5-7B reaches 90.0\% in English but
0--3\% in most other languages, indicating that the high English score is a
language-specific pattern match rather than a transferred capability. The
full per-language sub-task breakdown is in
Appendix~Table~\ref{tab:app_l3_subtask_lang}.

This sub-task structure has methodological implications: the aggregate L3
score in Table~\ref{tab:main_results} mixes genuine viewpoint-transformation
failure with metric ceiling effects on the boolean sub-task. We recommend
that follow-up work either drop \texttt{rotationCheck} from L3 aggregation
or apply a baseline-corrected scoring scheme.

\subsection{Reasoning Prompt Is Not a Universal Booster}
\label{sec:res_reasoning_prompt}

We instrument every (model, language, level) cell with two prompt regimes:
\emph{direct} (``answer the question'') and \emph{reasoning} (``think step
by step before answering''). The middle block of
Table~\ref{tab:cross_axis_summary} shows that the reasoning-prompt effect is
both model-dependent and level-dependent.

DeepSeek-V4-Flash gains the most: \textbf{+32.4} pp at L3 (10.2\% direct
$\to$ 42.7\% reasoning), with smaller positive gains across L0--L4.
Llama-3.1-8B also benefits at L0--L3 ($+$12 to $+$18 pp). Conversely,
GPT-4o, Gemini-2.5-Flash, Qwen2.5-7B, and Gemma all show \emph{negative}
deltas at L3--L5, with Qwen2.5-7B losing 15.6 pp at L3 and most
open-weight models losing 14--27 pp at L5. The L5 negative effect is
consistent with the hypothesis that chain-of-thought prompting disrupts
strict JSON output formatting: a model that emits a step-by-step
explanation before the JSON graph often produces a malformed JSON.

This pattern is paper-relevant for two reasons. First, it warns against
single-protocol benchmarks: reporting either direct-only or
reasoning-only would yield a different model ranking. Second, it suggests
that reasoning-prompt sensitivity itself is a diagnostic signal---models
that benefit substantially from the prompt (DeepSeek, Llama) appear to
have the latent capability but require explicit elicitation, while models
that lose accuracy under the prompt (Qwen2.5, Gemma at L5) may have
brittle output formatting that explicit reasoning destabilizes.

\subsection{Node Identification and Relation Extraction Dissociate at L5}
\label{sec:res_metric}

The right block of Table~\ref{tab:cross_axis_summary} reports L5 node F1
and edge F1 averaged across the four L5 sub-tasks. The two metrics
dissociate strongly for several models. Llama-3.1-8B achieves 87.4\% node
F1 but only 53.1\% edge F1---it identifies the objects in the scene but
fails to recover their containment relations. Mistral-7B and Falcon3-10B
show similar patterns (75.7/43.2 and 76.7/66.1 respectively). The
appendix Table~\ref{tab:app_l5_graph_diagnostics} expands these numbers
across the four L5 sub-tasks individually, revealing that the dissociation
is most pronounced on the \texttt{staticFocusedGraph} sub-task, where
Llama achieves 83.6\% node F1 but only 30.9\% edge F1.

Two corollaries follow. First, \textbf{strict pass rate at L5 is not
informative}: a response with the correct object set but wrong relations
fails strict matching entirely but earns substantial graph F1. We
therefore report partial-credit graph F1 as the L5 composite. Second,
\textbf{the strict-vs-partial dichotomy applies to L4 as well}: as the
left block of Table~\ref{tab:l4_counterfactual} shows, Falcon3-10B
achieves 53.8\% strict pass at L4 but only 5.6\% event precision,
indicating template-matching rather than genuine event tracking. This
dissociation suggests that benchmark composites must report at least two
metrics per task for the staircase to be honestly interpretable.

\input{tables/l4_counterfactual}

The right block of Table~\ref{tab:l4_counterfactual} shows the L5c
counterfactual case. Gemini-2.5-Flash achieves 83.3\% strict pass rate
but 0.0\% graph F1, the inverse pattern: it produces responses that
strict matching credits but the graph evaluator rejects as structurally
invalid. This case-by-case strict-vs-partial divergence reinforces the
methodological recommendation: \emph{report both metrics, on all levels,
for all benchmarks involving structured output}.

\subsection{Open-Weight Models Close the Gap Specifically at L5}
\label{sec:res_open_closed}

Across L0--L4 the closed-source group (GPT-4o, Gemini, DeepSeek) leads
the open-weight group by 5--26 pp on average (Table~\ref{tab:main_results}).
At L5, the gap reverses: averaged across L5 sub-tasks, the closed group
scores 65.3\% (GPT-4o 93.3, Gemini 31.6, DeepSeek 71.0) and the
open-weight group 66.4\% (Llama 62.0, Qwen2.5 73.8, Mistral 44.2,
Gemma 70.1, Falcon3 82.0, Qwen2.5-VL 66.4). The reversal is driven by
Gemini's catastrophic L5 performance and by strong L5 results from
Falcon3 and Gemma. We interpret this as a sign that generative
structured output---which couples natural-language understanding with
JSON formatting---is more sensitive to fine-tuning regime than to base
model scale, since several mid-scale open-weight models have evidently
been fine-tuned with strong JSON output supervision.

\subsection{Cross-Language Consistency Is Extremely Low}
\label{sec:res_multilingual}

\input{tables/belief_multilingual_hallucination}

The middle block of
Table~\ref{tab:belief_multilingual_hallucination} reports a strict
all-language-correct metric: the fraction of paired questions where
the model produces the correct answer in all eight evaluation languages
simultaneously. The numbers are striking. Even the strongest model on
this metric, Gemma-2-9B, only achieves 55.1\% all-language-correct at
L1, dropping to 1.7\% at L3 and 2.0\% at L5. GPT-4o (evaluated only on
L3--L5) achieves 3.4--13.9\% across those levels. The implication is
that current LLMs do not have a unified spatial understanding that
transfers across languages; rather, each language version of the task
is solved (or failed) somewhat independently.

This finding has a stronger version: \textbf{the existence of the L3
cliff in the average score may mask language-specific
near-monolingual cliffs in some models}. A model that scores 20\% at
L3 averaged across eight languages might be near-perfect in one
language and near-zero in seven; the all-language metric in
Table~\ref{tab:belief_multilingual_hallucination} reveals that this is
indeed the case for several models.

\subsection{Belief Revision Performs at Chance Level Across All Models}
\label{sec:res_belief}

The left block of Table~\ref{tab:belief_multilingual_hallucination}
reports the multi-turn belief-revision success rate, where round~2
introduces evidence contradicting the answer from round~1 and round~3
tests whether the model has correctly updated its spatial belief.
Almost all open-weight models cluster at \emph{exactly 20\%}---the
chance rate for a 5-option update---and the two with deviations are
Llama-3.1-8B (0\%, never revises) and Gemini-2.5-Flash (0\%, similar).
GPT-4o achieves 16.7\% and DeepSeek 20\%. The uniformity of the 20\%
result, combined with the small sample size per model (15--18 trials),
suggests that revision success is at or near chance and we cannot
distinguish model-level differences with the current protocol. This
finding is itself substantive: \textbf{none of the nine evaluated
models exhibits systematic belief revision on spatial state}. Larger
samples and longer-horizon protocols would be needed to test for
genuine revision capability, but the current chance-level result rules
out strong revision in this regime.

\subsection{Free-Form Hallucination Varies Dramatically with Output Format}
\label{sec:res_hallucination}

The right block of
Table~\ref{tab:belief_multilingual_hallucination} reports English
free-form hallucination on the L5 hallucination-focused sub-task,
where the model is asked to list scene objects in free-form text rather
than structured JSON. Eight of nine models achieve near-perfect object
F1, indicating that they do not hallucinate phantom objects when output
format is unconstrained. The exception is Gemini-2.5-Flash, which
produces empty or non-listing responses on this sub-task (objF1 0\%,
24 missing objects). The contrast with the structured-output L5
sub-tasks in Table~\ref{tab:app_l5_graph_diagnostics} is striking: the
same models that produce 0--30\% missing nodes on free-form output
produce 5--380 missing nodes on structured graph output. \textbf{The
hallucination/omission failure mode is therefore not a model-level
property but an output-format-coupled property.} This complements the
Section~\ref{sec:res_reasoning_prompt} finding that explicit reasoning
disrupts structured output: both findings point to a fragility in how
current LLMs translate between natural-language understanding and
structured world-graph emission.


==> sections/06_discussion.tex <==
\section{Discussion}
\label{sec:discussion}

The seven findings argue against treating spatial reasoning as a single capability. Failure modes are \emph{structural} (frame confusion, anchor flips, node--edge dissociations) rather than arithmetic, and the Kendall's $\tau$ discontinuity at the static-to-active boundary ($+0.50\!\to\!+0.18$) shows per-language rankings reorganize across tiers. F7 supplies the strongest reading: \emph{across all eight languages}, native speakers collapse to L3$=$0\% while L4 plateaus at $\sim$41\% (std 3.3pp)---a cross-lingual replication that rules out language-specific accounts and points at the modality. The implied mechanism is a verbal working-memory bottleneck \citep{cowan2001magical}, compatible with probing evidence that LLMs encode partial spatial structure internally \citep{li2024probing,vafa2024evaluating}.


==> tables/belief_multilingual_hallucination.tex <==
% =============================================================================
% Table 7 (main paper): Belief revision + Multilingual consistency + Free-form
% hallucination, all in one dense table. Each axis is one column-group.
%
% Supports findings:
%   - §5.5 Belief revision is at chance level across all models
%   - §5.6 Multilingual consistency is extremely low even on top models
%   - §5.7 Free-form hallucination is rare in English but varies elsewhere
% =============================================================================

\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l cc | cccccc | ccc}
\toprule
& \multicolumn{2}{c|}{\textbf{Belief revision (en)}}
& \multicolumn{6}{c|}{\textbf{Multilingual consistency (all-8-languages-correct \%)}}
& \multicolumn{3}{c}{\textbf{Free-form hallucination (en)}} \\
\textbf{Model}
& \textbf{revSucc\%} & \textbf{n}
& \textbf{L0} & \textbf{L1} & \textbf{L2} & \textbf{L3} & \textbf{L4} & \textbf{L5}
& \textbf{objF1\%} & \textbf{hallucObj} & \textbf{missObj} \\
\midrule
\rowcolor{blue!10}
\multicolumn{12}{l}{\textbf{\textit{(A) Frontier closed-source}}} \\
GPT-4o             & 16.7 & 18  &  --  &  --  &  --  & 3.4  & 13.9 & 6.9  & 100.0 & 0.00 & 0.00 \\
Gemini-2.5-Flash   & 0.0  & 8   &  --  &  --  &  --  & 0.0  & 0.7  & 0.0  & 0.0   & 0.00 & 24.00 \\
DeepSeek-V4-Flash  & 20.0 & 15  & 26.4 & 54.7 & 14.5 & 0.3  & 12.2 & 2.2  & 100.0 & 0.00 & 0.00 \\
\midrule
\rowcolor{orange!10}
\multicolumn{12}{l}{\textbf{\textit{(B) Open-weight (7--10B)}}} \\
Llama-3.1-8B       & 0.0  & 15  & 4.9  & 10.9 & 8.3  & 0.0  & 3.6  & 0.0  & 100.0 & 0.00 & 0.00 \\
Qwen2.5-7B         & 20.0 & 15  & 19.5 & 12.6 & 7.7  & 0.1  & 7.3  & 0.2  & 100.0 & 0.00 & 0.00 \\
Mistral-7B         & 20.0 & 15  & 5.6  & 1.3  & 6.0  & 0.0  & 5.0  & 0.0  & 100.0 & 0.00 & 0.00 \\
Gemma-2-9B         & 20.0 & 15  & 26.2 & 55.1 & 12.3 & 1.7  & 18.7 & 2.0  & 100.0 & 0.00 & 0.00 \\
Falcon3-10B        & 20.0 & 15  & 0.1  & 10.3 & 1.8  & 0.0  & 3.1  & 0.0  & 100.0 & 0.00 & 0.00 \\
Qwen2.5-VL-3B      & 7.8  & 90  & 15.1 & 5.4  & 5.7  & 0.0  & 4.6  & 0.0  & 98.2  & 0.00 & 0.61 \\
\bottomrule
\end{tabular}%
}
\caption{
\label{tab:belief_multilingual_hallucination}
\textbf{Belief revision, multilingual consistency, and English hallucination
diagnostics.}
\emph{Left}: revision-success rate on a 3-turn conflict protocol where round~2
contradicts round~1 (en, direct prompt). Nearly all models cluster around
20\% (1/5), indicating that none performs systematic belief revision; the
finding is consistent with chance-level behavior on a 5-option update.
\emph{Middle}: fraction of paired questions where the model answers
correctly in \emph{all eight} evaluation languages simultaneously
(higher = better cross-lingual consistency). The metric is extremely low
across all models---even Gemma-2-9B, the best open-weight model on this
axis, achieves only 55.1\% all-language-correct at L1 and drops to 1.7\% at
L3. \emph{Right}: free-form scene-listing hallucination (en): eight of nine
models achieve near-perfect object F1, the exception being Gemini-2.5-Flash
which omits scene objects almost entirely in its free-form output.
GPT-4o and Gemini-2.5-Flash were not evaluated on L0--L2 multilingual cells.
}
\end{table*}

